From Nilspace Theory to Simplicial Homotopy Theory

We construct a faithful functor from the category of cubespaces, arising in structured ergodic theory and nilspace theory, to the category of (condensed) simplicial sets. This functor translates the weak structure theorem of a nilspace to a Postnikov tower of the corresponding simplicial set. In particular, nilspaces are mapped to Kan complexes and the structure groups of the nilspace correspond to the simplicial homotopy groups of the Kan complex. The functor is constructed via pullback along a special cosimplicial cubical set, whose combinatorial properties may be of independent interest.

==> macros.tex <==
\hfuzz 100pt % lässt die overfull hbox warnings verschwinden
\newcommand{\noa}[1]{~{\color{red}Noa: #1}}
\newcommand{\nick}[1]{~{\color{blue}Nick: #1}}

%%
%% Packages
%%

\usepackage{xltabular} % bessere Tabellen
\usepackage{comment} % für Kommentare
\usepackage{scalerel} % richtige Skalierung der speziellen Kategorienzeichen
\RequirePackage{enumerate}
\RequirePackage{mathrsfs}
\RequirePackage{euscript}
\usepackage[shortlabels]{enumitem}
\usepackage{array,longtable,booktabs,cancel,ragged2e,multirow}
\usepackage{titlesec} % Titelanpassungen
\RequirePackage[autostyle=true]{csquotes}
\usepackage{graphicx,wrapfig}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{quiver} % kommutative Diagramme

%%
%% Categories
%%

\newcommand{\fin}{\mathrm{Fin}}
\let\Fin\fin
\newcommand{\finert}{{\operatorname{Fin}_{\ast,\mathrm{inert}}}}
\newcommand{\inert}{{\bbGamma_{\ast,\mathrm{inert}}}}
\newcommand{\set}{\mathrm{Set}}
\let\Set\set
\newcommand{\Ab}{\mathrm{Ab}}
\newcommand{\Grp}{\mathrm{Grp}}
\newcommand{\Ring}{\mathrm{Ring}}
\newcommand{\Mod}{\mathrm{Mod}} % \Mod_R
\newcommand{\ModR}{\Mod_R}
\newcommand{\Vect}{\mathrm{Vect}} % \Vect(\R), \Vect_n(\R)
\newcommand{\Mon}{\mathrm{Mon}}
\newcommand{\cMon}{\mathrm{CMon}}
\newcommand{\bool}{\mathrm{Bool}}
\newcommand{\sbool}{\mathrm{Bool}_\sigma}
\newcommand{\cbool}{\mathrm{Bool}_{\mathrm{comp}}}

\newcommand{\Ani}{\mathrm{Ani}}

\newcommand{\Top}{\mathrm{Top}}
\newcommand{\stone}{\mathrm{Stone}}
\newcommand{\CHaus}{\mathrm{CHaus}}
\newcommand{\extr}{\mathrm{Extr}}
\newcommand{\prof}{\Pro(\Fin)}
\newcommand{\prolak}{\prof_\kappa}
\newcommand{\LCA}{\mathrm{LCA}}

\newcommand{\sSet}{\mathrm{sSet}}
\newcommand{\sAb}{\mathrm{sAb}}

\newcommand{\Cat}{\mathrm{Cat}}
\newcommand{\PrL}{\mathrm{Pr}^\mathrm{L}}

\newcommand{\cond}{\mathrm{Cond}}
\let\Cond\cond
\newcommand{\CondSet}{\mathrm{CondSet}}
\newcommand{\CondAni}{\mathrm{CondAni}}
\newcommand{\cAb}{\mathrm{CondAb}}
\newcommand{\CondAb}{\mathrm{CondAb}}
\newcommand{\CondRing}{\mathrm{CondRing}}
\newcommand{\CondMod}{\mathrm{CondMod}}
\newcommand{\qcqs}{\mathrm{qcqs}}
\newcommand{\liq}{\mathrm{liq}}
\newcommand{\MMp}{\mathcal{M}_{<p}}

\newcommand{\cSet}{\mathrm{cSet}}
\newcommand{\ccSet}{\mathrm{cSet}^\mathrm{conc}}
\newcommand{\cSetnil}{{\mathrm{cSet}_\mathrm{fib}}}
\newcommand{\ccSetnil}{\mathrm{cSet}_\mathrm{fib}^\mathrm{conc}}
\newcommand{\cCond}{\mathrm{cCond}}


%%
%% Operators
%%

\newcommand{\Id}{\operatorname{Id}}
\newcommand{\id}{\operatorname{id}}

\newcommand{\subobj}{\operatorname{Sub}}
\newcommand{\su}{\operatorname{Sub}_{\bbDelta}}

\newcommand{\Gprod}{{\prod^{\mathrm{Gray}}}}
\newcommand{\ev}{\operatorname{ev}}
\newcommand{\Bun}{\operatorname{Bun}}
\newcommand{\HK}{\operatorname{HK}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\PSh}{\operatorname{PSh}}
\newcommand{\Sh}{\mathrm{Sh}}
\newcommand{\EM}{\operatorname{EM}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Pro}{\operatorname{Pro}}
\newcommand{\sInd}{\operatorname{sInd}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\Lan}{\operatorname{Lan}}
\newcommand{\Ran}{\operatorname{Ran}}
\newcommand{\Coim}{\operatorname{coim}}
\newcommand{\Ch}{\operatorname{Ch}}
\newcommand{\tot}{\operatorname{tot}}
\newcommand{\co}{\operatorname{co}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\divop}{\operatorname{div}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\esssup}{\operatorname{ess\,sup}}
\newcommand{\essrang}{\operatorname{ess\,rang}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\fix}{\operatorname{fix}}
\renewcommand{\gcd}{\operatorname{gcd}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\interior}{\operatorname{int}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\orb}{\operatorname{orb}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\diag}{\operatorname{diag}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\cosk}{\operatorname{cosk}}
\newcommand{\sing}{\operatorname{Sing}}
\newcommand{\cof}{\operatorname{cof}}

\newcommand{\im}{\operatorname{im}}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Cov}{\operatorname{Cov}}

\newcommand{\Hom}{\operatorname{Hom}}
\let\hom\Hom
\newcommand{\ihom}{\underline{\hom}}
\newcommand{\iHom}{\underline{\hom}}
\newcommand{\Rhom}{\operatorname{RHom}}
\newcommand{\RHom}{\Rhom}
\newcommand{\iRHom}{\underline{\Rhom}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\iExt}{\underline{\Ext}}
\newcommand{\Iso}{\operatorname{Iso}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Trans}{\operatorname{Trans}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Mat}{\operatorname{Mat}} % \Mat(n, m; \R), \Mat_n(\R)
\newcommand{\Mor}{\operatorname{Mor}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\GL}{\operatorname{GL}} % \GL(n, \R)
\newcommand{\SL}{\operatorname{SL}} % \SL(n, \R)
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Alt}{\operatorname{Alt}}
\newcommand{\Bil}{\operatorname{Bil}}
\newcommand{\Gal}{\operatorname{Gal}} % \Gal(E/F)

\newcommand{\Ob}{\mathrm{Ob}}
\newcommand{\ob}{\Ob}
\newcommand{\op}{\mathrm{op}}
\newcommand{\from}{\leftarrow}

%%
%% Letters
%%

\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cX{\mathcal{X}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}

\newcommand\mcA{\cA}
\newcommand\mcB{\cB}
\newcommand\mcC{\cC}
\newcommand\mcD{\cD}
\newcommand\mcE{\cE}
\newcommand\mcF{\cF}
\newcommand\mcG{\cG}
\newcommand\mcH{\cH}
\newcommand\mcI{\cI}
\newcommand\mcJ{\cJ}
\newcommand\mcK{\cK}
\newcommand\mcL{\cL}
\newcommand\mcM{\cM}
\newcommand\mcN{\cN}
\newcommand\mcO{\cO}
\newcommand\mcP{\cP}
\newcommand\mcQ{\cQ}
\newcommand\mcR{\cR}
\newcommand\mcS{\cS}
\newcommand\mcT{\cT}
\newcommand\mcU{\cU}
\newcommand\mcV{\cV}
\newcommand\mcW{\cW}
\newcommand\mcX{\cX}
\newcommand\mcY{\cY}
\newcommand\mcZ{\cZ}

\newcommand{\ua}{\mathrm{a}}
\newcommand{\ub}{\mathrm{b}}
\newcommand{\uc}{\mathrm{c}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\uf}{\mathrm{f}}
\newcommand{\ug}{\mathrm{g}}
\newcommand{\uh}{\mathrm{h}}
\newcommand{\ui}{\mathrm{i}}
\newcommand{\uj}{\mathrm{j}}
\newcommand{\uk}{\mathrm{k}}
\newcommand{\ul}{\mathrm{l}}
\newcommand{\um}{\mathrm{m}}
\newcommand{\un}{\mathrm{n}}
\newcommand{\uo}{\mathrm{o}}

\AtBeginDocument{
  \ifdefined\up
    \let\frup\up
    \renewcommand{\up}{\mathrm{p}}
  \else
    \newcommand{\up}{\mathrm{p}}
  \fi
}
\newcommand{\uq}{\mathrm{q}}
\newcommand{\ur}{\mathrm{r}}
\newcommand{\us}{\mathrm{s}}
\newcommand{\ut}{\mathrm{t}}
\newcommand{\uu}{\mathrm{u}}
\newcommand{\uv}{\mathrm{v}}
\newcommand{\uw}{\mathrm{w}}
\newcommand{\ux}{\mathrm{x}}
\newcommand{\uy}{\mathrm{y}}
\newcommand{\uz}{\mathrm{z}}

\newcommand{\uA}{\mathrm{A}}
\newcommand{\uB}{\mathrm{B}}
\newcommand{\uC}{\mathrm{C}}
\newcommand{\uD}{\mathrm{D}}
\newcommand{\uE}{\mathrm{E}}
\newcommand{\uF}{\mathrm{F}}
\newcommand{\uG}{\mathrm{G}}
\newcommand{\uH}{\mathrm{H}}
\newcommand{\uI}{\mathrm{I}}
\newcommand{\uJ}{\mathrm{J}}
\newcommand{\uK}{\mathrm{K}}
\newcommand{\uL}{\mathrm{L}}
\newcommand{\uM}{\mathrm{M}}
\newcommand{\uN}{\mathrm{N}}
\newcommand{\uO}{\mathrm{O}}
\newcommand{\uP}{\mathrm{P}}
\newcommand{\uQ}{\mathrm{Q}}
\newcommand{\uR}{\mathrm{R}}
\newcommand{\uS}{\mathrm{S}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uU}{\mathrm{U}}
\newcommand{\uV}{\mathrm{V}}
\newcommand{\uW}{\mathrm{W}}
\newcommand{\uX}{\mathrm{X}}
\newcommand{\uY}{\mathrm{Y}}
\newcommand{\uZ}{\mathrm{Z}}


\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\F}{\mathbb{F}}
\renewcommand{\S}{\mathbb{S}}
\renewcommand{\O}{\mathcal{O}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\bS}{\mathbf{S}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\fM}{\mathfrak{M}}

%%
%% Measures
%%

\newcommand{\da}{\,\mathrm{d}a}
\newcommand{\db}{\,\mathrm{d}b}
\newcommand{\dc}{\,\mathrm{d}c}
\newcommand{\dd}{\,\mathrm{d}d}
\newcommand{\de}{\,\mathrm{d}e}
\newcommand{\df}{\,\mathrm{d}f}
\newcommand{\dg}{\,\mathrm{d}g}
\newcommand{\di}{\,\mathrm{d}i}
\newcommand{\dk}{\,\mathrm{d}k}
\newcommand{\dl}{\,\mathrm{d}l}
\newcommand{\dm}{\,\mathrm{d}m}
\newcommand{\dn}{\,\mathrm{d}n}
\newcommand{\dr}{\,\mathrm{d}r}
\newcommand{\ds}{\,\mathrm{d}s}
\newcommand{\dt}{\,\mathrm{d}t}
\newcommand{\du}{\,\mathrm{d}u}
\newcommand{\dv}{\,\mathrm{d}v}
\newcommand{\dw}{\,\mathrm{d}w}
\newcommand{\dx}{\,\mathrm{d}x}
\newcommand{\dy}{\,\mathrm{d}y}
\newcommand{\dz}{\,\mathrm{d}z}

\newcommand{\dalpha}{\,\mathrm{d}\alpha}
\newcommand{\dbeta}{\,\mathrm{d}\beta}
\newcommand{\dgamma}{\,\mathrm{d}\gamma}
\newcommand{\ddelta}{\,\mathrm{d}\delta}
\newcommand{\depsilon}{\,\mathrm{d}\epsilon}
\newcommand{\dzeta}{\,\mathrm{d}\zeta}
\newcommand{\deta}{\,\mathrm{d}\eta}
\newcommand{\dtheta}{\,\mathrm{d}\theta}
\newcommand{\diota}{\,\mathrm{d}\iota}
\newcommand{\dkappa}{\,\mathrm{d}\kappa}
\newcommand{\dlambda}{\,\mathrm{d}\lambda}
\newcommand{\dmu}{\,\mathrm{d}\mu}
\newcommand{\dnu}{\,\mathrm{d}\nu}
\newcommand{\dxi}{\,\mathrm{d}\xi}
% No \omikron because it's the same as a plain o.
\newcommand{\dpi}{\,\mathrm{d}\pi}
\newcommand{\drho}{\,\mathrm{d}\rho}
\newcommand{\dsigma}{\,\mathrm{d}\sigma}
\newcommand{\dtau}{\,\mathrm{d}\tau}
\newcommand{\dupsilon}{\,\mathrm{d}\upsilon}
\newcommand{\dphi}{\,\mathrm{d}\phi}
\newcommand{\dchi}{\,\mathrm{d}\chi}
\newcommand{\dpsi}{\,\mathrm{d}\psi}
\newcommand{\domega}{\,\mathrm{d}\omega}

\newcommand{\dA}{\,\mathrm{d}A}
\newcommand{\dB}{\,\mathrm{d}B}
\newcommand{\dC}{\,\mathrm{d}C}
\newcommand{\dD}{\,\mathrm{d}D}
\newcommand{\dE}{\,\mathrm{d}E}
\newcommand{\dF}{\,\mathrm{d}F}
\newcommand{\dG}{\,\mathrm{d}G}
\newcommand{\dH}{\,\mathrm{d}H}
\newcommand{\dI}{\,\mathrm{d}I}
\newcommand{\dJ}{\,\mathrm{d}J}
\newcommand{\dK}{\,\mathrm{d}K}
\newcommand{\dL}{\,\mathrm{d}L}
\newcommand{\dM}{\,\mathrm{d}M}
\newcommand{\dN}{\,\mathrm{d}N}
\newcommand{\dO}{\,\mathrm{d}O}
\newcommand{\dP}{\,\mathrm{d}P}
\newcommand{\dQ}{\,\mathrm{d}Q}
\newcommand{\dR}{\,\mathrm{d}R}
\newcommand{\dS}{\,\mathrm{d}S}
\newcommand{\dT}{\,\mathrm{d}T}
\newcommand{\dU}{\,\mathrm{d}U}
\newcommand{\dV}{\,\mathrm{d}V}
\newcommand{\dW}{\,\mathrm{d}W}
\newcommand{\dX}{\,\mathrm{d}X}
\newcommand{\dY}{\,\mathrm{d}Y}
\newcommand{\dZ}{\,\mathrm{d}Z}

\let\oldforall\forall
\let\oldexists\exists
\renewcommand{\forall}{\,\oldforall\,}
\renewcommand{\exists}{\,\oldexists\,}

% "Geschmackssache.", sagte der Affe und biss in die Seife.

\let\subob\leq
\let\supob\geq
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\newcommand{\oldleq}{\subob}
\newcommand{\oldgeq}{\supob}

% \varepsilon is _way_ cooler than \epsilon.

\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\varepsilon}
\let\eps\epsilon
\let\oldphi\phi
\renewcommand{\phi}{\varphi}
\let\oldtheta\theta
\renewcommand{\theta}{\vartheta}

% Either use \subseteq or \subsetneq, \subset is not needed and misguiding.
% bei Nick gibts kein \subseteq, das ist einfach notational overload

%\renewcommand{\subset}{\subseteq}
%\renewcommand{\supset}{\supseteq}
\newcommand{\sub}{\subseteq}

% correctly typesets := and =:
\newcommand{\defeq}{\mathrel{\vcentcolon=}}
\newcommand{\eqdef}{\mathrel{=\vcentcolon}}

% Creates a version of \mid that can (only) be used between
% \left and \right and scales correctly.
\newcommand{\mmid}{\,\middle|\,}

% Dots for parameters, to be used if f(\cdot) doesn't cut it
\newcommand{\pardot}{{}\mathbin{\cdot}{}}

\newcommand{\smallboxtimes}{\mathbin{\XBox}}

\renewcommand{\tilde}[1]{\widetilde{#1}}
\renewcommand{\hat}[1]{\widehat{#1}}


\let\longimplies\implies
\renewcommand{\implies}{\longimplies}

\newcommand{\myqedsymbol}{\ensuremath{\Box}}

% In case a proof doesn't work out as planned (requires tikz)

\newcommand{\semiqed}{
  \parfillskip=0pt\nobreak\hfill
  {
    \scalebox{0.5}{
    \def\sqedlength{0.25}
    \def\sqedlength{0.5}
    \begin{tikzpicture}[overlay]
      \draw[densely dashed](0.0, 0.0) -- (0.0, \sqedlength);
      \draw[densely dashed](0.0, \sqedlength) -- (\sqedlength, \sqedlength);
      \draw[densely dashed](\sqedlength, \sqedlength) -- (\sqedlength, 0.0);
      \draw[densely dashed](0.0, 0.0) -- (\sqedlength, 0.0);
    \end{tikzpicture}
      }
  }\hspace{2px}
  \par
}

\newcounter{proofstep}
\newcommand{\step}[1][]{
  \refstepcounter{proofstep}
  \ifthenelse{\equal{#1}{}}{%
    %omitted
    \par\textbf{\mystepname\,\theproofstep:}
  }{%supplied
    \par\textbf{\mystepname\,\theproofstep\,{\normalfont(#1)}:}\unskip
  }
}

%%% \vvvert (|||x||| Norm), copied from https://tex.stackexchange.com/a/193126
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}
\DeclareFontSubstitution{U}{matha}{m}{n}

% Math symbol font mathb
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}

% Symbol definition
\DeclareMathDelimiter{\vvvert}{0}{matha}{"7E}{mathx}{"17}


%

\DeclareRobustCommand{\bbDelta}{% blackboard bold Delta
	\mathchoice{\Delta\llap{\scalebox{0.775}{$\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\scriptstyle\Delta$\hspace{0.025em}}}}%
	{\Delta\llap{\scalebox{0.775}{$\scriptscriptstyle\Delta$\hspace{0.025em}}}}
	}

\DeclareRobustCommand{\bbGamma}{% blackboard bold Gamma
	\mathchoice{\raisebox{\depth}{\scalebox{1}[-1]{$\mathbb L$}}}%
	{\raisebox{\depth}{\scalebox{1}[-1]{$\mathbb L$}}}%
	{\raisebox{\depth}{\scalebox{1}[-1]{$\scriptstyle\mathbb L$}}}%
	{\raisebox{\depth}{\scalebox{1}[-1]{$\scriptscriptstyle\mathbb L$}}}
	}

% Symbol für die Cube Kategorie

\makeatletter
\newcommand{\bbsquaretikz}{%
    \mathrel{%
        \scalerel*{%
            \tikz[scale=0.23, line cap=round, baseline=-0.04ex]{%
                \draw[line width=.8pt, rounded corners=.1pt] (0,0) rectangle (1,1);
                \draw[line width=.3pt] (0.2,0) -- (0.2,1);
            }
        }{\square}
    }
}
\makeatother

\DeclareMathOperator*{\bbox}{\bbsquaretikz}

% Symbol für die lineare Cube Kategorie

\makeatletter
\newcommand{\bblsquaretikz}{%
    \mathrel{%
        \scalerel*{%
            \tikz[scale=0.23, line cap=round, baseline=-0.04ex]{%
                \draw[line width=.8pt, rounded corners=.1pt] (0,0) rectangle (1,1);
                \draw[line width=.3pt] (0.2,0.2) -- (0.2,1);
                \draw[line width=.3pt] (0.2,0.2) -- (1,0.2);
            }
        }{\square}
    }
}
\makeatother

\DeclareMathOperator*{\bblox}{\bblsquaretikz}

% Symbol für die Ecke

\makeatletter
\newcommand{\bbcornertikz}{%
    \mathrel{%
        \scalerel*{%
            \tikz[scale=0.23, line cap=round, baseline=-0.04ex]{%
                \draw[line width=.8pt] (0,0) -- (1,0);
                \draw[line width=.8pt] (0,0) -- (0,1);
                \draw[line width=.3pt] (0.2,0.2) -- (0.2,1);
                \draw[line width=.3pt] (0.2,0.2) -- (1,0.2);
            }
        }{\square}
    }
}
\makeatother

\DeclareMathOperator*{\bbcor}{\bbcornertikz}

%

%prisma eventuell so
\makeatletter
\newcommand{\bprism}{%
  \mathord{%
    \vcenter{\hbox{%
      \tikz[scale=0.25, line cap=round, line join=round]{%
        % back triangle
        \draw[line width=.35pt]
          (0.45,0.25) -- (1.35,0.25) -- (0.90,1.05) -- cycle;
        % connecting edges
        \draw[line width=.35pt]
          (0,0) -- (0.45,0.25);
        \draw[line width=.35pt]
          (0.90,0) -- (1.35,0.25);
        \draw[line width=.35pt]
          (0.45,0.80) -- (0.90,1.05);
        % front triangle
        \draw[line width=.35pt, rounded corners=.1pt]
          (0,0) -- (0.90,0) -- (0.45,0.80) -- cycle;
      }%
    }}%
  }%
}
\makeatother

%

\newcommand*\lon{%    % das umgedrehte \colon
        \nobreak
        \mskip6mu plus1mu
        \mathpunct{}%
        \nonscript
        \mkern-\thinmuskip
        {:}%
        \mskip2mu
        \relax
}

%

% Compact labelled 3-cube macro.
%
% Usage:
% \smallcube{Name}
%   {top-left}{top-right}
%   {upper-left}{upper-right}
%   {middle-left}{middle-right}
%   {bottom-left}{bottom-right}
%
% The macro draws at the current TikZ origin, so place it inside a scope:
% \begin{scope}[shift={(2.5,0)}]
%   \smallcube{C_3^4}{12}{123}{12}{13}{02}{023}{012}{013}
% \end{scope}

\tikzset{
  smallcube edge/.style={
    draw=black!55,
    line width=0.35pt,
    line cap=round,
    shorten <=1.5pt,
    shorten >=1.5pt
  },
  smallcube label/.style={
    font=\scriptsize,
    inner sep=0.7pt,
    fill=white
  },
  smallcube name/.style={
    font=\scriptsize\bfseries,
    anchor=south
  }
}

\newcommand{\smallcube}[9]{%
  \coordinate (smallcubeBL) at (0,0);
  \coordinate (smallcubeBR) at (1.45,0);
  \coordinate (smallcubeML) at (0.48,0.68);
  \coordinate (smallcubeMR) at (1.93,0.68);
  \coordinate (smallcubeUL) at (0,1.36);
  \coordinate (smallcubeUR) at (1.45,1.36);
  \coordinate (smallcubeTL) at (0.48,2.04);
  \coordinate (smallcubeTR) at (1.93,2.04);

  \node[smallcube name] at (0.96,2.35) {$#1$};

  \draw[smallcube edge] (smallcubeTL) -- (smallcubeTR);
  \draw[smallcube edge] (smallcubeTL) -- (smallcubeML);
  \draw[smallcube edge] (smallcubeTR) -- (smallcubeMR);
  \draw[smallcube edge] (smallcubeUL) -- (smallcubeTL);
  \draw[smallcube edge] (smallcubeUL) -- (smallcubeUR);
  \draw[smallcube edge] (smallcubeUL) -- (smallcubeBL);
  \draw[smallcube edge] (smallcubeUR) -- (smallcubeTR);
  \draw[smallcube edge] (smallcubeBL) -- (smallcubeML);
  \draw[smallcube edge] (smallcubeBL) -- (smallcubeBR);
  \draw[smallcube edge] (smallcubeBR) -- (smallcubeUR);
  \draw[smallcube edge] (smallcubeBR) -- (smallcubeMR);
  \draw[smallcube edge] (smallcubeML) -- (smallcubeMR);

  \node[smallcube label] at (smallcubeTL) {$#2$};
  \node[smallcube label] at (smallcubeTR) {$#3$};
  \node[smallcube label] at (smallcubeUL) {$#4$};
  \node[smallcube label] at (smallcubeUR) {$#5$};
  \node[smallcube label] at (smallcubeML) {$#6$};
  \node[smallcube label] at (smallcubeMR) {$#7$};
  \node[smallcube label] at (smallcubeBL) {$#8$};
  \node[smallcube label] at (smallcubeBR) {$#9$};
}

%

\allowdisplaybreaks[2] % encourages pagebreaks in formulas multiple lines long
                       % NOTE: Does not work with align, alignat, ... but e.g.
                       % with align*.

\theoremstyle{plain}

\newtheorem{theorem}{Theorem}[subsection]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

% German stuff

\newtheorem{satz}[theorem]{Satz}
\newtheorem{folgerung}[theorem]{Folgerung}

\theoremstyle{definition}

\newtheorem{reminder}[theorem]{Reminder}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{warning*}[theorem]{Warning}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{note}[theorem]{Note}
\newtheorem{motivation}[theorem]{Motivation}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{definition}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}

\newtheorem{exercise}{Exercise}[subsection]

\newtheorem{example}[theorem]{Example}
\newtheorem{construction}[theorem]{Construction}

% unnumbered environments

\theoremstyle{plain}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{proposition*}{Proposition}
\newtheorem*{conjecture*}{Conjecture}

\newtheorem*{satz*}{Satz}
\newtheorem*{folgerung*}{Folgerung}

\theoremstyle{remark}

\newtheorem*{reminder*}{Reminder}
\newtheorem*{remark*}{Remark}
\newtheorem*{notation*}{Notation}
\newtheorem*{motivation*}{Motivation}
\newtheorem*{assumption*}{Assumption}

\theoremstyle{definition}

\newtheorem*{definition*}{Definition}
\newtheorem*{question*}{Question}
\newtheorem*{problem*}{Problem}
\newtheorem*{exercise*}{Exercise}
\newtheorem*{example*}{Example}
\newtheorem*{construction*}{Construction}

\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta}

\newcommand{\bigrtimes}{%
  \mathop{\scalerel*{\rtimes}{\sum}}\displaylimits
}

%%
%% Theorems etc. in der Einleitung nach hinten referenzieren
%%

\makeatletter

\newenvironment{repeatresult}[2]{%
  \begingroup

  % Save environment name and label for the closing part
  \def\repeatresult@env{#1}%
  \def\repeatresult@label{#2}%

  % Save theorem machinery
  \let\repeatresult@origbegintheorem\@begintheorem
  \let\repeatresult@origopargbegintheorem\@opargbegintheorem
  \let\repeatresult@origrefstepcounter\refstepcounter

  % Do not increment a counter for the repeated statement
  \def\refstepcounter##1{}%

  % hyperref patches theorem counters separately
  \@ifundefined{Hy@theorem@refstepcounter}{}{%
    \let\repeatresult@orighyrefstepcounter\Hy@theorem@refstepcounter
    \def\Hy@theorem@refstepcounter##1{}%
  }%

  % Replace the displayed theorem number by the referenced number
  \def\@begintheorem##1##2{%
    \repeatresult@origbegintheorem
      {##1}{\ref{\repeatresult@label}}%
  }%

  \def\@opargbegintheorem##1##2##3{%
    \repeatresult@origopargbegintheorem
      {##1}{\ref{\repeatresult@label}}{##3}%
  }%

  % Start theorem / lemma / proposition / ...
  \csname #1\endcsname

  % Restore normal machinery for the theorem body
  \let\refstepcounter\repeatresult@origrefstepcounter

  \@ifundefined{repeatresult@orighyrefstepcounter}{}{%
    \let\Hy@theorem@refstepcounter\repeatresult@orighyrefstepcounter
  }%

  \let\@begintheorem\repeatresult@origbegintheorem
  \let\@opargbegintheorem\repeatresult@origopargbegintheorem
}{%
  \csname end\repeatresult@env\endcsname
  \endgroup
}

\makeatother


